On successive minima-type inequalities for the polar of a convex body

Motivated by conjectures of Mahler and Makai Jr., we study bounds on the volume of a convex body in terms of the successive minima of its polar body.

==> macros_math.tex <==
%\renewcommand{\labelenumi}{\rm \roman{enumi})}
\renewcommand{\Re}{\mathrm{Re}} %real part
\renewcommand{\Im}{\mathrm{Im}} %imaginary part

%\def\I#1{\mathrm{I}_{\,#1}} %identity matrix
\newcommand{\I}{\mathrm{I}}

\newcommand{\sa}{\mathrm{a}}
\newcommand{\Le}{\mathrm{g}}
\newcommand{\LE}{\mathrm{G}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\V}{\mathrm{V}} %intrinsic volumes
\newcommand{\F}{\mathrm{F}} %surface area
\newcommand{\U}{\mathrm{U}} %U-functional
\newcommand{\W}{\mathrm{W}} %mixed volumes
\newcommand{\bor}{\mathrm{b}\,}
\newcommand{\ir}{\mathrm{r}} %inradius
\newcommand{\cR}{\mathrm{R}} %circumradius
\newcommand{\di}{\mathrm{D}} %diameter
\newcommand{\dbm}{\mathrm{d}_{\rm BM}} %Banach-Mazur distance
\newcommand{\iso}{\mathrm{L}}
\newcommand{\dlat}{\mathrm{d}}
\newcommand{\diff}{\mathrm{D}}%Difference body
\newcommand{\e}{\mathrm{e}}
\newcommand{\w}{\mathrm{w}}
\newcommand{\LL}{\mathrm{L}}
\newcommand{\DV}{\mathrm{DV}}

\newcommand{\ggT}{\mathrm{ggT}\, } %german gcd
\newcommand{\kgV}{\mathrm{kgV}\, } %german lcm
\newcommand{\GL}{\mathrm{GL}} %general linear group
\newcommand{\SL}{\mathrm{SL}} %special linear group
\newcommand{\grad}{\mathrm{grad}}
\newcommand{\schsym}{{\mathrm S}_L} %Schwarz-symmetral
\newcommand{\inte}{\mathrm{int}\,}  %interior of a set
\newcommand{\relint}{\mathrm{relint}\,}  %relinterior of a set
\newcommand{\cl}{\mathrm{cl}\,} %closure
\newcommand{\bd}{\mathrm{bd}\,} %boundary
\newcommand{\relbd}{\mathrm{relbd}\,} %rel boundary
\newcommand{\aff}{\mathrm{aff}\,} %affine hull
\newcommand{\conv}{\mathrm{conv}\,} %convex hull
\newcommand{\diag}{\mathrm{diag}\,} %diagonal matrix
\newcommand{\dist}{\mathrm{dist}\,} %distance
\newcommand{\epi}{\mathrm{epi}\,} %epigraph
\DeclareMathOperator{\lin}{lin}
\DeclareMathOperator{\linz}{lin_\Z}
%\newcommand{\lin}{\mathrm{lin}} %linear hull
\newcommand{\pos}{\mathrm{pos}\,} %positive hull
\newcommand{\sgn}{\mathrm{sgn}\,} %sign
\newcommand{\st}{\mathrm{st}}
\newcommand{\tra}{\mathrm{tr}} %trace of a matrix
\newcommand{\verte}{\mathrm{vert}\,} %I guess for vertices
\newcommand{\vol}{\mathrm{vol}\,} %well, volume


\newcommand{\grass}{\mathcal{G}} %grassmannian
\newcommand{\grassz}{\mathcal{G}_\Z} %grassmannian of lattice planes 
\newcommand{\Lat}{\mathcal{L}} % lattice
\newcommand{\latp}[1]{\left|\, #1 \,\right|}
\newcommand{\cKn}{\mathcal{K}_0^n} %old definition of 0-symmetric convex bodies in \R^n
\newcommand{\B}{\mathcal{B}}
\newcommand{\Kn}{{\mathcal K}^n} %convex bodies
\newcommand{\Cn}{{\mathcal C}^n}
\newcommand{\Pn}{{\mathcal P}^n} %polytopes
\newcommand{\Kon}{{\mathcal K}_o^n} %o-symmetric convex bodies
\newcommand{\Ksn}{{\mathcal K}_{(s)}^n} %o-symmetric convex bodies
\newcommand{\Knull}{{\mathcal K}_{(o)}^n} %o-symmetric convex bodies
\newcommand{\Kcn}{{\mathcal K}_c^n} %centered convex bodies, centroid
                                %at 0
\newcommand{\E}{{\mathcal E}} %ellipsoid
\newcommand{\packset}{\mathcal{P}} %packing set
\newcommand{\facet}{\mathcal{F}}
\newcommand{\pack}{\mathcal{P}}
\newcommand{\packl}{\mathcal{P}_\Lat}

\newcommand{\R}{\mathbb{R}} %real numbers
\newcommand{\Ss}{\mathbb{S}}
\newcommand{\N}{\mathbb{N}} %natural numbers
\newcommand{\Z}{\mathbb{Z}} %integral numbers
\newcommand{\Q}{\mathbb{Q}} %rational numbers
\newcommand{\C}{\mathbb{C}} %complex numbers
\newcommand{\K}{\mathbb{K}} %fields

\newcommand{\bo}{\mathfrak{B}}
\newcommand{\gmh}{\mathfrak{H}}


\newcommand{\abs}[1]{{\left|#1\right|}} %absoulte value of a number

\newcommand{\norm}[2]{\left\vert #1\right\vert_{#2}} %general norm with respect to a body
\newcommand{\enorm}[1]{\left\lvert #1\right\rvert} %Euclidean norm
\newcommand{\onorm}[1]{\left\lvert #1\right\rvert_1}
\newcommand{\pnorm}[1]{\Vert #1\Vert_p}

\newcommand{\disuni}{\mathbin{\setbox0\hbox{$\bigcup$}\rlap{\copy0}\raise.3%
  \ht0\hbox to \wd0{\hfil$\cdot$\hfil}}}
  
\newcommand{\ip}[2]{\left\langle #1,#2\right\rangle}
%\newcommand{\ip}[2]{ #1^\intercal\, #2}

\newcommand{\dual}[1]{{#1}^\star}
\newcommand{\Cpds}{C_{\rm pds}} %Cone of definite positive matrices
\newcommand{\ov}{\overline}
\newcommand{\gso}[1]{\overline{#1}}
\newcommand{\alg}[2]{{#1}^{_{(#2)}}}

%-----------------------------------------
\newcommand{\ban}{B_n}
\newcommand{\bani}[1]{B_{#1}}
\newcommand{\denl}{\delta_\Lat}
\newcommand{\otau}{\overline{\tau}}
\newcommand{\trans}{\intercal}
\newcommand{\tr}{\intercal} %transpose

\newcommand{\bx}{{\vx}}
\newcommand{\by}{{\vy}}
\newcommand{\bz}{{\vz}}
\newcommand{\ba}{{\va}}
\newcommand{\bb}{{\vb}}
\newcommand{\bc}{{\vc}}
\newcommand{\bl}{{\vl}}
\newcommand{\bp}{{\vp}}
\newcommand{\bq}{{\vq}}
%\newcommand{\bs}{{\vs}}
\newcommand{\bu}{{\vu}}
%\newcommand{\bm}{{\vm}}
\newcommand{\bn}{{\vn}}
\newcommand{\bt}{{\vt}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\be}{{\ve}}

%boldsymbols for vectors
\newcommand{\va}{{\boldsymbol a}}
\newcommand{\vb}{{\boldsymbol b}}
\newcommand{\vc}{{\boldsymbol c}}
\newcommand{\ve}{{\boldsymbol e}}
\newcommand{\vs}{{\boldsymbol s}}
\newcommand{\vt}{{\boldsymbol t}}
\newcommand{\vl}{{\boldsymbol l}}
\newcommand{\vu}{{\boldsymbol u}}
\newcommand{\vv}{{\boldsymbol v}}
\newcommand{\vw}{{\boldsymbol w}}
\newcommand{\vx}{{\boldsymbol x}}
\newcommand{\vy}{{\boldsymbol y}}
\newcommand{\vz}{{\boldsymbol z}}
\newcommand{\vh}{{\boldsymbol h}}
\newcommand{\vg}{{\boldsymbol g}}
\newcommand{\vm}{{\boldsymbol m}}
\newcommand{\vone}{{\boldsymbol 1}}
\newcommand{\vlambda}{{\boldsymbol \lambda}}
\newcommand{\vnull}{{\boldsymbol 0}}
\newcommand{\vq}{{\boldsymbol q}}


\newcommand{\bA}{{\boldsymbol A}}
\newcommand{\bB}{{\boldsymbol B}}
\newcommand{\bC}{{\boldsymbol C}}
\newcommand{\bD}{{\boldsymbol D}}
\newcommand{\bI}{{\boldsymbol I}}
\newcommand{\bL}{{\boldsymbol L}}
\newcommand{\bT}{{\boldsymbol T}}
\newcommand{\bM}{{\boldsymbol M}}
\newcommand{\bU}{{\boldsymbol U}}
\newcommand{\bV}{{\boldsymbol V}}
\newcommand{\bX}{{\boldsymbol X}}

%-------------------------------




%beamer 
% \definecolor{author}{rgb}{0.5,0.5,0.0}
% \definecolor{defcol}{rgb}{0.0,0.5,0.5}
% \definecolor{def}{rgb}{0.0,0.5,0.5}
% \definecolor{highcol}{rgb}{0.1,0.2,0.5}
 %\definecolor{high}{rgb}{0.1,0.2,0.5}


\newcommand{\Hl}{H_{\leq}}
\newcommand{\Hg}{H_{\geq}}
\newcommand{\dha}{\mathrm{d}_{\rm H}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\Lamp}{\Lambda^\circ}
\newcommand{\mahler}{\mathrm{M}\,} %Mahler volume
\newcommand{\cs}{\mathrm{cs}\,}%central symmetral
\newcommand{\cPn}{\mathcal{P}_o^n}% 0-symmetric polytopes


\newcommand{\hermite}{\mathrm{h}}

\newcommand{\Mn}{\mathcngeschränkte Aal{M}^n}


\newcommand{\suk}{\mathrm{h}}%support fnction
\newcommand{\width}{\mathrm{w}}% width 
\newcommand{\diam}{\mathrm{D}}%diameter


\newcommand{\recc}{\mathrm{rec}\,} % recession cone
\newcommand{\ext}{\mathrm{ext}\,} % extreme points
%\newcommand{\exp}{\mathrm{exp}\,} % exposed points
\newcommand{\extr}{\mathrm{extr}\,} % extreme rays
\newcommand{\vbeta}{{\boldsymbol \beta}}
\newcommand{\vphi}{{\boldsymbol \phi}}
%\newcommand{\vphi}{{\boldsymbol \phi}}
\newcommand{\sar}{\mathrm{S}}
\newcommand{\dive}{\mathrm{div}}

\newcommand{\VP}{\mathrm{VP}} %general linear group
%\newcommand{\SL}{\mathrm{SL}} %special linear group det =1 
\newcommand{\OR}{\mathrm{O}} % orthognal matrices O^\tran O = I_n


\newcommand{\vor}{\mathrm{DV}} %Dirichlet-Voronoi cell 

\newcommand{\sph}{\mathbb{S}}% sphere

\newcommand{\cen}{\mathrm{c}}%centroid

\newcommand{\vora}{\mathrm{vr}}%volume ratio }

\newcommand{\bone}{\mathbf{1}}

\newcommand{\prob}{\mathbb{P}}
\newcommand{\med}{\mathrm{med}} %median 
\newcommand{\sm}{\mu}% notation of the probabilty measure on the
                           % sphere..
\newcommand{\Ex}{\mathbb{E}} % expectation

\newcommand{\supp}{\mathrm{supp}} % support 

\newcommand{\lwidth}{\mathrm{w}} % lattice width 

